Who is Responsible? Explaining Safety Violations in Multi-Agent Cyber-Physical Systems

Multi-agent cyber-physical systems are present in a variety of applications. Agent decision-making can be affected due to errors induced by uncertain, dynamic operating environments or due to incorrect actions taken by an agent. When an erroneous decision that leads to a violation of safety is identified, assigning responsibility to individual agents is a key step toward preventing future accidents. Current approaches to carrying out such investigations require human labor or high degree of familiarity with operating environments. Automated strategies to assign responsibility can achieve a significant reduction in human effort and associated cognitive burden. In this paper, we develop an automated procedure to assign responsibility for safety violations to actions of any single agent in a principled manner. We base our approach on reasoning about safety violations in road safety. Given a safety violation, we use counterfactual reasoning to create alternative scenarios, showing how different outcomes could have occurred if certain actions had been replaced by others. We introduce the degree of responsibility (DoR) metric for each agent. The DoR, using the Shapley value, quantifies each agent's contribution to the safety violation, providing a basis to explain and justify decisions. We also develop heuristic techniques and methods based on agent interaction structures to improve scalability as agent numbers grow. We examine three safety violation cases from the National Highway Traffic Safety Administration (NHTSA). We run experiments using CARLA urban driving simulator. Results show the DoR improves the explainability of decisions and accountability for agent actions and their consequences.

==> appdendix.tex <==
\newpage
\appendix

\subsection{Proof of Proposition \ref{prop:monotone}}\label{app:monotone}

Consider two counterfactual worlds $\mathcal{C}_\mathcal{Y}^t$ and $\mathcal{C}_{\mathcal{Y}'}^t$.
When $\mathcal{Y}=\mathcal{Y}'$, then the proposition trivially holds.
We prove the proposition holds for $\mathcal{Y}\subset\mathcal{Y}'$ by contradiction.
We assume that Eq. \eqref{eq:monotone} does not hold in this case.
In this case, we have that $\mathcal{Y}'\setminus\mathcal{Y}\neq\emptyset$.
We denote the policies taken by each agent $i\in\mathcal{Y}'\setminus\mathcal{Y}$ as $\pi_i'$.
We thus have 
\begin{equation}\label{eq:contradiction}
    r(C_{\mathcal{Y}'}^t;\{\pi_i'\}_{i\in\mathcal{Y}}\cup\{\pi_i'\}_{i\in\mathcal{Y}'\setminus\mathcal{Y}},\tilde{\pi}')>r(C_\mathcal{Y}^t;\{\pi_i\}_{i\in\mathcal{Y}},\tilde{\pi}).
\end{equation}
Eq. \eqref{eq:contradiction}, however, contradicts the definition of the utility function in Eq. \eqref{eq:reward}, where $\{\pi_i'\}_{i\in\mathcal{Y}'\setminus\mathcal{Y}}$ should minimize the probability of reaching the unsafe states.
Indeed, the agents in $\mathcal{Y}\subset\mathcal{Y}'$ can take the actions as observed in path $\rho$ to obtain a lower probability of violating the safety constraint based on the hypothesis.
Therefore, we have that Eq. \eqref{eq:monotone} must hold, which completes our proof.

% \subsection{Proof of Proposition \ref{prop:DoR}}\label{app:DoR}
% By Proposition \ref{prop:monotone}, we have that $u(\mathcal{Y}\cup\{i\})-u(\mathcal{Y})\leq 0$.
% Since $\phi_i$ in Eq. \eqref{eq:phi} is a linear combination of $u(\mathcal{Y}\cup\{i\})-u(\mathcal{Y})$ with positive coefficients, the value of $\phi_i$ satisfies $\phi_i\leq 0$ for all $i\in\mathcal{N}$.
% Note that the DoR in Eq. \eqref{eq:dor} is obtained by normalizing $\phi_i$ over all agents, we have that the proposition holds.

\subsection{Proof of Lemma \ref{lemma:local Q}}\label{app:zero stage local Q}

For any joint state $s\in\mathcal{S}$ and action $a\in\mathcal{A}$, we have
\begin{align}
    &\left|Q^L(s_i^{\mathcal{B}^k},a_i^{\mathcal{B}^k},0)-Q(s,a,0)\right|\nonumber\\
    =&\Bigg|\sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)\nonumber\\
    &\quad\quad\cdot Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}),0\right) -Q(s,a,0)\Bigg|\label{eq:approx bound-1}\\
    &\Bigg|\sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)\nonumber\\
    &\quad\quad\cdot Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}),0\right) \nonumber\\
    &-\sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)Q(s,a,0)\Bigg|\label{eq:approx bound-2}\\
    &\leq \sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)\nonumber\\
    &\quad\quad\quad\quad\Big|Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}),0\right) \nonumber\\
    &\quad\quad\quad\quad\quad\quad- Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^{k'}}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^{k'}}),0\right)\Big|\label{eq:approx bound-3}\\
    \leq &c\gamma^{k+1},\label{eq:approx bound-4}
\end{align}
where Eq. \eqref{eq:approx bound-1} holds by the definition of local Q-function in Eq. \eqref{eq:local Q}, Eq. \eqref{eq:approx bound-2} holds by Eq. \eqref{eq:weight}, Eq. \eqref{eq:approx bound-3} follows by rearranging Eq. \eqref{eq:approx bound-2} and applying the definition $s$ and $a$, and Eq. \eqref{eq:approx bound-4} holds by Definition \ref{def:exponential decay relaxed}.

% \begin{align}
%     &\left|Q^L(s_i^{\mathcal{B}^k},a_i^{\mathcal{B}^k},t)-Q(s,a,t)\right|\nonumber\\
%     =&\Bigg|\sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)\nonumber\\
%     &\quad\quad\cdot Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right) -Q(s,a,t)\Bigg|\label{eq:approx bound-1}\\
%     &\Bigg|\sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)\nonumber\\
%     &\quad\quad\cdot Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right) \nonumber\\
%     &-\sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)Q(s,a,t)\Bigg|\label{eq:approx bound-2}\\
%     &\leq \sum_{s_{-i}^{\mathcal{B}^k}\in\mathcal{S}_{-i}^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}\omega_i\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k})\right)\nonumber\\
%     &\quad\quad\quad\quad\Big|Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}),t\right) \nonumber\\
%     &\quad\quad\quad\quad\quad\quad- Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^{k'}}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^{k'}}),t\right)\Big|\label{eq:approx bound-3}\\
%     \leq &c\gamma^{k+1},\label{eq:approx bound-4}
% \end{align}
% where Eq. \eqref{eq:approx bound-1} holds by the definition of local Q-function in Eq. \eqref{eq:local Q}, Eq. \eqref{eq:approx bound-2} holds by Eq. \eqref{eq:weight}, Eq. \eqref{eq:approx bound-3} follows by rearranging Eq. \eqref{eq:approx bound-2} and applying the definition $s$ and $a$, and Eq. \eqref{eq:approx bound-4} holds by Definition \ref{def:exponential decay}.







\subsection{Proof of Proposition \ref{prop:local Q}}\label{app:local Q optimality}

% This is a relaxed version of Definition \ref{def:exponential decay}.
% \begin{definition}[$(c,\gamma)$ Exponential Decay Property]\label{def:exponential decay relaxed}
%     The $(c,\gamma)$ exponential decay property holds for some $c>0$ and $\gamma\in(0,1)$ if the following inequality holds
%     \begin{multline}
%         \Big|Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}),0\right) \\
%         - Q\left((s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^{k'}}),(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^{k'}}),0\right)\Big|
%         \leq c\gamma^{k+1}
%     \end{multline}
%     for any agent $i\in\mathcal{N}$, joint states $(s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^k}), (s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^{k'}})\in\mathcal{S}$, and joint actions $(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^k}), (a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^{k'}})\in\mathcal{A}$.
% \end{definition}


% Given Definition \ref{def:exponential decay}, we show that we can approximate the Q-function using the local Q-function for any stage $t$.
% \begin{proposition}\label{prop:local Q}
%     Let $s=(s_i^{\mathcal{B}^k},s_{-i}^{\mathcal{B}^{k'}})\in\mathcal{S}$ and $a=(a_i^{\mathcal{B}^k},a_{-i}^{\mathcal{B}^{k'}})\in\mathcal{A}$ be the joint state and action of the MMDP $\mathbb{M}$. 
%     If the MMDP $\mathbb{M}$ satisfies the $(c,\gamma)$ exponential decay property in Definition \ref{def:exponential decay}, then for any stage $t=0,\ldots,T-1$, the following relationship holds
%     \begin{equation}
%         \sup_{s_{-i}^{\mathcal{B}^{k'}}\in\mathcal{S}_{-i}^{\mathcal{B}^{k'}},a_{-i}^{\mathcal{B}^k}\in\mathcal{A}_{-i}^{\mathcal{B}^k}}|Q^L(s_i^{\mathcal{B}^k},a_i^{\mathcal{B}^k},t)-Q(s,a,t)|\leq c\gamma^{k+1}.
%     \end{equation}
% \end{proposition}

    We prove the proposition by induction. 
    The induction base is given in Definition \ref{def:exponential decay relaxed}.
    Assume that the proposition holds for stage $t'=0,\ldots,t-1$. 
    In the following, we prove that the proposition holds for stage $t$.
    We have 
    \begin{align}
    &\left|Q^L(s_i^{\mathcal{B}^k},a_i^{\mathcal{B}^k},t)-Q(s,a,t)\right|\nonumber\\
    =&\Bigg|\sum_{s_i^{\mathcal{B}^{k'}}\in\mathcal{S}_i^{\mathcal{B}^k}}Pr^L\left(s_i^{\mathcal{B}^{k'}}|s_i^{\mathcal{B}^k},a_i^{\mathcal{B}^k}\right)\min_{a'}Q(s_i^{\mathcal{B}^{k'}},a_i^{\mathcal{B}^{k'}},t-1)\nonumber\\
    &\quad\quad-\sum_{s'\in\mathcal{S}}Pr(s'|s,a)\min_{a'}Q(s',a',t-1)
    \Bigg|\label{eq:approx bound relax-1}\\
    \leq & \sum_{s'\in\mathcal{S}}Pr(s'|s,a)|Q(s_i^{\mathcal{B}^{k'}},a_i^{\mathcal{B}^{k'}},t-1) - Q(s',a',t-1)|\label{eq:approx bound relax-2}\\
    &\leq c\gamma^{k+1}\label{eq:approx bound relax-3}
    \end{align}
where Eq. \eqref{eq:approx bound relax-1} holds by Eq. \eqref{eq:local Q update} and \eqref{eq:Q-value 2}, Eq. \eqref{eq:approx bound relax-2} holds by Eq. \eqref{eq:marginal transition prob} and the triangle inequality, and  and Eq. \eqref{eq:approx bound relax-3} holds by our induction hypothesis.


\subsection{Proof of Theorem \ref{thm:DoR bound}}\label{app:DoR bound}

Consider an agent $i\in\mathcal{N}$.
We denote the value of Eq. \eqref{eq:utility} evaluated using Q-function and local Q-function as $u$ and $u^L$, respectively.
Using the definitions of $\phi_i$ and $\phi_i^L$, we have
\begin{align}
    &|\phi_i-\phi_i^L|\nonumber\\
    =&\Bigg|\frac{1}{|\mathcal{N}|}\sum_{\mathcal{Y}\subseteq\mathcal{N}\setminus\{i\}}{\mathcal{N}\choose |\mathcal{N}|-|\mathcal{Y}|-1}^{-1}\Big[u(\mathcal{Y}\cup\{i\})-u(\mathcal{Y})\nonumber\\
    &\quad\quad\quad\quad\quad\quad-(u^L(\mathcal{Y}\cup\{i\})-u^L(\mathcal{Y}))\Big]\Bigg|\label{eq:DoR bound-1}\\
    =&\Bigg|\frac{1}{|\mathcal{N}|}\sum_{\mathcal{Y}\subseteq\mathcal{N}\setminus\{i\}}{\mathcal{N}\choose |\mathcal{N}|-|\mathcal{Y}|-1}^{-1}\Big[u(\mathcal{Y}\cup\{i\})\nonumber\\
    &\quad\quad\quad\quad-u^L(\mathcal{Y}\cup\{i\})+u^L(\mathcal{Y}) -u(\mathcal{Y})\Big]\Bigg|\label{eq:DoR bound-2}\\
    \leq&\frac{1}{|\mathcal{N}|}\sum_{\mathcal{Y}\subseteq\mathcal{N}\setminus\{i\}}{\mathcal{N}\choose |\mathcal{N}|-|\mathcal{Y}|-1}^{-1}\Big[ |u^L(\mathcal{Y}) -u(\mathcal{Y})|\nonumber\\
    &\quad\quad\quad\quad+|u(\mathcal{Y}\cup\{i\})-u^L(\mathcal{Y}\cup\{i\})|\Big]\label{eq:DoR bound-3}\\
    \leq&\frac{1}{|\mathcal{N}|}\sum_{\mathcal{Y}\subseteq\mathcal{N}\setminus\{i\}}2{\mathcal{N}\choose |\mathcal{N}|-|\mathcal{Y}|-1}^{-1}c\gamma^{k+1},\label{eq:DoR bound-4}\\
    =&c^L\gamma^{k+1}\label{eq:DoR bound-5}
\end{align}
where Eq. \eqref{eq:DoR bound-1} holds by the definitions of $\phi_i$ and $\phi_i^L$, Eq. \eqref{eq:DoR bound-2} holds by rearranging Eq. \eqref{eq:DoR bound-1}, Eq. \eqref{eq:DoR bound-3} follows from the triangle inequality, Eq. \eqref{eq:DoR bound-4} holds by Proposition \ref{prop:local Q}, and Eq. \eqref{eq:DoR bound-5} holds by the definition of $c^L$.

==> discussion.tex <==
\section{This is for Discussion Purpose}

\textbf{Challenge of Algorithm 3:} One challenge of Algorithm 3 is the choice of quantifier in line 6. Note that the safe policies come as tuples. In other words, a safe policy $\pi_i^1$ may not form another safe policy $(\pi_1^k,\ldots,\pi_i^1,\ldots,\pi_N^k)$. Therefore, it is possible that $P(u_i^0,\ldots,u_i^T;\pi_i)< \epsilon$ holds for some safe policy $\pi$ for all agent $i$, leading to no responsible agents.
If we change the quantifier to `existence', then we may classify some innocent agents to be responsible. 


\begin{center}
  	\begin{algorithm}[!htp]
  		\caption{Another Version of Identification of Responsible Agents}
  		\label{algo:identify}
  		\begin{algorithmic}[1]
  			\State \textbf{Input}: The set of agents $\mathcal{V}$ who violated safety constraint, the paths $\{\rho_i\}_{i\in\mathcal{N}}$ and actions $\{u_i^t\}_{i\in\mathcal{N},t=1,\ldots,T}$ took by all agents, thershold $\epsilon$ 
  			\State \textbf{Output:} The set of responsible agents $\mathcal{R}\subseteq\mathcal{N}$
            \State \textbf{Initialize:} $\mathcal{R}\leftarrow\emptyset$
            \State Compute a set of $K$ numbers safe policies for all agents $\boldsymbol{\pi}=\{(\pi_1^1,\ldots,\pi_N^1), (\pi_1^2,\ldots,\pi_N^2), \ldots, (\pi_1^K,\ldots,\pi_N^K)\}$ \Comment{Safe policy computation is a optimal control problem on MMDP}
            \For{$i\in\mathcal{N}$}
            \If{$P(u_i^0,\ldots,u_i^T;\pi_i)< \epsilon$ holds for all safe policies $\pi\in\boldsymbol{\pi}$ \Comment{\textcolor{blue}{What should be quantifier here?}}} 
            \State $\mathcal{R}\leftarrow\mathcal{R}\cup\{i\}$
            \EndIf
            \EndFor
            \State \textbf{Return} $\mathcal{R}$
  		\end{algorithmic}
  	\end{algorithm}
\end{center}


==> prelim.tex <==
\section{Preliminary Background}\label{sec:preliminaries}

In this section, we present the preliminary background on coalitional games and the Shapley value.

A coalitional game can be used to model the interaction among a set of decision makers (also known as players).
A coalition is defined as follows.
\begin{definition}[Coalition \cite{fudenberg1991game}]
    Give a set of players $\mathcal{N}$, a \emph{coalition} is a nonempty subset of $\mathcal{N}$. 
    The set $\mathcal{N}$ itself is called the \emph{grand coalition}.
\end{definition}
A coalitional game is then formally defined as follows.
\begin{definition}[Coalitional Game \cite{fudenberg1991game}]\label{def:coalitional game}
    A coalitional game is a pair $(\mathcal{N},u)$, where $\mathcal{N}$ is a finite set of players, and $u:2^{\mathcal{N}}\rightarrow\mathbb{R}$ is a real-valued  utility function.
\end{definition}
The utility function in Definition \ref{def:coalitional game} represents the utility of any coalition $\mathcal{Y}\subseteq\mathcal{N}$, which can be distributed among the members of coalition $\mathcal{Y}$. 
The Shapley value \cite{roth1988shapley} is one solution concept to distribute the utility of a coalition. 
In particular, given a coalitional game $(\mathcal{N},u)$, the Shapley value assigns each player $\phi_i$ amount of payoff to each player $i\in\mathcal{N}$, where 
\begin{equation}\label{eq:shapley}
    \phi_i = \frac{1}{|\mathcal{N}|}\sum_{\mathcal{Y}\subseteq\mathcal{N}\setminus\{i\}}{\mathcal{N}\choose |\mathcal{N}|-|\mathcal{Y}|-1}^{-1}(u(\mathcal{Y}\cup\{i\})-u(\mathcal{Y})).
\end{equation}
Intuitively, the Shapley value considers all possible orders in which the players can join a coalition, and defines the payoff of player $i$ as its marginal contribution, i.e., $u(\mathcal{Y}\cup\{i\})-u(\mathcal{Y})$, averaged over all possible orders.

==> sol_backup.tex <==
\section{Solution Approach}

\subsection{Overview}

Our solution approach consists of two components: \emph{identification of responsible agents} and \emph{DoR quantification}.

\subsection{Computation of Safe Policies}

Since we focus on the MMDP setting, it suffices to consider deterministic policies. 
Note that since we consider finite time horizon, the optimal policy may not be stationary.

We define a value function $v^t(s)$ for all $s\in\mathcal{S}$ to represent $t$-stage-to-go probability of reaching the unsafe states $\hat{\mathcal{S}}$ when starting from $s$.
By the Bellman equation, we have
\begin{equation}
    v^{t}(s) = \min_{u\in A(s)}\sum_{s'\in \mathcal{S}}Pr(s'|s,u)v^{t-1}(s')
\end{equation}
Then the optimal policy $\pi(s)^{t,*}=(\pi_1^{t,*}(s_1),\ldots,\pi_N^{t,*}(s_N))$ on MMDP can be found as 
\begin{equation}
    \pi^{t,*}(s)\in\arg\min_u\sum_{s'\in \mathcal{S}}Pr(s'|s,u) v^{t-1}(s).
\end{equation}
To find the set of safe polices such that Eq. \eqref{eq:safety} holds, we can compute the Q-values for all joint state-action pairs, and use $\delta$ as the threshold to filter out the safe policies.
% We denote the optimal value for the value function function as $v^{T,*}\in\mathbb{R}^{|\mathcal{S}|}$.
% Since the agents may be \emph{bounded rational}, we consider a policy $\pi$ to be a \emph{safe policies} if $v^{T,*}\leq \min\{\delta,v^{T,*}+\lambda\}$, where $\lambda$ models the level of bounded rationality.
% We denote the set of safe policies as $\boldsymbol{\pi}$.

\subsection{Identification of Responsible Agents}

This component is to identify the set of clients $\mathcal{R}\subseteq\mathcal{N}$ such that $\phi_i>0$ for all $i\in\mathcal{R}$ and $\phi_i=0$ for all $i\notin \mathcal{R}$.

We denote $\mathcal{V}\subseteq\mathcal{N}$ as the set of agents who violated the safety constraint. 
That is, the agent $i\in\mathcal{V}$ took some action $u_i^t$ that led to some transition from $s_i^t$ to $s_i^{t+1}$ satisfying $c(s_i^t,s_i^{t+1})>0$.  

We use Algorithm \ref{algo:identify} to identify the set of responsible agents.
The algorithm takes $\mathcal{V}$, the paths of all agents, and a threshold $\epsilon$ as inputs.
It outputs the set of responsible agents $\mathcal{R}\subseteq\mathcal{N}$.
The algorithm first initializes $\mathcal{R}$ as an empty set.
It then computes a set of safe policies $\boldsymbol{\pi}_i$ for each agent $i\in\mathcal{V}$, assuming that the agents in $\mathcal{N}\setminus\mathcal{V}$ follow the same actions that they have taken in the path.
This problem can be formulated as an optimal control problem on an MMDP, where the actions of agents in $\mathcal{N}\setminus\mathcal{V}$ and initial states of agents in $\mathcal{N}$ are given.
If $\boldsymbol{\pi}_i$ is non-empty, we then verify the probability that the agent $i$ takes the sequence of actions in the path under each policy $\pi_i\in\boldsymbol{\pi}_i$, denoted as $P(u_i^0,\ldots,u_i^t;\pi_i)$.
If $P(u_i^0,\ldots,u_i^t;\pi_i)<\epsilon$ for all policy $\pi_i$, then it is likely that the agent followed an unsafe policy.
Therefore, it should be responsible for the safety violation, and thus is included in $\mathcal{R}$.
If there is no safe policy for some agent $i$, we then verify whether the safety violation is triggered by some agent $j\in\mathcal{N}\setminus\mathcal{V}$.
We next compute the safe policies for agent $i$ by removing some agents $\mathcal{W}$ from $\mathcal{N}\setminus\mathcal{V}$, until there exists some safe policy for agent $i$.
In this case, the agents in $\mathcal{W}$ that was removed last time will be included in $\mathcal{R}$.



\begin{center}
  	\begin{algorithm}[!htp]
  		\caption{Identification of Responsible Agents}
  		\label{algo:identify}
  		\begin{algorithmic}[1]
  			\State \textbf{Input}: The set of agents $\mathcal{V}$ who violated safety constraint, the paths $\{\rho_i\}_{i\in\mathcal{N}}$ and actions $\{u_i^t\}_{i\in\mathcal{N},t=1,\ldots,T}$ took by all agents, thershold $\epsilon$ 
  			\State \textbf{Output:} The set of responsible agents $\mathcal{R}\subseteq\mathcal{N}$
            \State \textbf{Initialize:} $\mathcal{R}\leftarrow\emptyset$
            \State Assume the agents in $\mathcal{N}\setminus\mathcal{V}$ take the same actions as observed in the path, compute a set of safe policies $\boldsymbol{\pi}_i$ for each agent in $\mathcal{V}$ \Comment{Safe policy computation is a optimal control problem on MMDP}
            \For{$i\in\mathcal{V}$}
            \If{ $\boldsymbol{\pi}_i\neq\emptyset$ \Comment{There exists some safe policy $\pi_i$}}
            \If{$P(u_i^0,\ldots,u_i^T;\pi_i)< \epsilon$ holds $\forall \pi_i\in\boldsymbol{\pi}_i$ \Comment{The agent's actions deviated from all safe policies}} 
            \State $\mathcal{R}\leftarrow\mathcal{R}\cup\{i\}$
            \EndIf
            \Else
            \While{$\boldsymbol{\pi}_i=\emptyset$}
            \State Remove some agents $\mathcal{W}$ from $\mathcal{N}\setminus\mathcal{V}$ \Comment{In the worst-case, we may need to iterate over all possible subsets of $\mathcal{N}\setminus \mathcal{V}$}
            \State Compute a set of safe policies $\boldsymbol{\pi}_i$ for each agent in $\mathcal{V}$, assuming all agents in $\mathcal{N}\setminus(\mathcal{V}\cup\mathcal{W})$ follow the same actions
            \EndWhile
            \State $\mathcal{R}\leftarrow\mathcal{R}\cup\mathcal{W}$ \Comment{agent $j$ may trigger the unsafe behavior of agent $i$, although agent $j$ did not violate safety constraint}
            \EndIf
            \EndFor
            \State \textbf{Return} $\mathcal{R}$
  		\end{algorithmic}
  	\end{algorithm}
\end{center}

\textcolor{blue}{A challenge is how to solve the optimal control problem in line 4? The actual state space could be larger than the states traversed along the paths of all agents. Therefore, the policies for agents at the non-traversed states remain undefined.}

One way to resolve this is to assume that the agents will follow a safe policy for the states that are not included in the observed path.

\textcolor{blue}{A challenge is how to solve the problem in line 12? We probably want some minimal subset $\mathcal{W}$ in $\mathcal{N}\setminus\mathcal{V}$ such that $\boldsymbol{\pi}_i$ becomes non-empty.}


We develop the following algorithm to compute $\mathcal{W}$.
Suppose that we cannot find a safe policy for agent $i\in\mathcal{V}$.
We define $u_{-i}$ as $u_{-i}=(u_1,\ldots,u_{i-1},u_{i+1},\ldots,u_N)$ and $s_{-i\setminus j}=(s_1,\ldots,s_{i-1},s_{i+1},\ldots,s_{j-1},s_{j+1},\ldots,s_N)$.
For each state $s_i$ and an admissible action $u_i\in A(s_i)$, we compute a set $\mathcal{L}$.
We then search for the states $\mathcal{L}=\{s:c(s,s')>0,Pr(s'|s,(\pi_i,u_{-i}))>0\}$, where $u_{-i}=(u_1,\ldots,u_{i-1},u_{i+1},\ldots,u_N)$.
Starting from $\mathcal{L}$ and taking action $u_i$ leads to non-zero costs, assuming the other agents take the actions that have been observed.
We next compute the set $\mathcal{W}(s_i)$ as $\mathcal{W}(s_i) =\{j\in\mathcal{N}:c((s_i,s_{-i\setminus j}),(s_i',s_{-i\setminus j}'))Pr((s_i',s_{-i\setminus j}')|(s_i,s_{-i\setminus j}),(u_i,u_{-i\setminus j}))=0\}$.
Finally, $\mathcal{W}$ is calculated as the intersection of all $\mathcal{W}(s_i)$.



\begin{center}
  	\begin{algorithm}[!htp]
  		\caption{Compute set $\mathcal{W}$}
  		\label{algo:identify}
  		\begin{algorithmic}[1]
  			\State \textbf{Input}: Agent $i$ who cannot find a safe policy
  			\State \textbf{Output:} The set of responsible agents $\mathcal{W}$ who did not violate $\mathcal{R}\subseteq\mathcal{N}$
            \For{$s_i\in\mathcal{S}_i$ and $u_i\in A(s_i)$}
            
            \State $\mathcal{L}\leftarrow\ \mathcal{L}\cup\{s:c((s_i,s_{-i}),(s_i',s_{-i}'))>0,Pr((s_i',s_{-i}')|(s_i,s_{-i}),(u_i,u_{-i}))>0\}$ \Comment{The set of states leads to non-zero costs}
            \State $\mathcal{W}(s_i)\leftarrow\{j\in\mathcal{N}:c((s_i,s_{-i\setminus j}),(s_i',s_{-i\setminus j}'))Pr((s_i',s_{-i\setminus j}')|(s_i,s_{-i\setminus j}),(u_i,u_{-i\setminus j}))=0\}$
            \EndFor
            \State $\mathcal{W}\leftarrow \cap_{s_i\in\mathcal{S}_i}\mathcal{W}(s_i)$
            \State \textbf{Return} $\mathcal{W}$
  		\end{algorithmic}
  	\end{algorithm}
\end{center}




\subsection{DoR Quantification}

DoR quantification characterizes to what extent each agent in $\mathcal{R}$ is responsible to the safety violation. 
Given the paths of all agents, we then have the information on the cost associated with the safety violation, denoted as $C$.
Our idea is to split the total cost $C$ among the agents in $\mathcal{R}$ using Shapley value.

For any subset of agents $\mathcal{Y}\subseteq\mathcal{R}$, we define a cost function as 
\begin{equation}
    Q(\mathcal{Y}) = \min_{\pi_i:i\in\mathcal{Y}}\left\{\mathbb{E}_{\mathcal{Y}}\left[\sum_{t=0}^{T-1} c(s^t,s^{t+1})\right] \right\}
\end{equation}

\begin{eqnarray}
    Q(\mathcal{Y}) = \sum_{t=0}^{T-1}{\min_{\pi_{i} : i \in \mathcal{N}}}{\mathbf{E}\left[\sum_{t^{\prime}=t}^{T-1}{c(s^{t^{\prime}},s^{t^{\prime}+1}) | s^{t} = \hat{s}^{t}, a_{t}^{i} = \pi_{i}(\hat{s}^{t}) \ \forall i \in \mathcal{Y}, } \right.}\\
    \left.a_{t}^{i} = \hat{a}_{t}^{i} \ \forall i \notin \mathcal{Y}, a_{t^{\prime}}^{i} = \pi_{i}(s^{t^{\prime}}) \ \forall t^{\prime} > t\right]
\end{eqnarray}

where the expectation $\mathbb{E}_{\mathcal{Y}}$ is taken with respect to the safe policies $\pi_i$ taken by the agents in $\mathcal{Y}$ and the transition probabilities, assuming that the agents in $\mathcal{R}\setminus \mathcal{Y}$ follow their actions that have been taken.
The cost function $Q(\mathcal{Y})$ captures (1) the cost incurred on MMDP when the agents in $\mathcal{Y}$ switch to safe policies, and (2) the cost for the agents in $\mathcal{Y}$ to switch to the safe policy.

\textcolor{blue}{Note that the term $\sum_{i\in\mathcal{Y}} \sum_{s_i\in \mathcal{S}_i}\|\pi_i(s_i)-u_i\|$ is NOT well-defined. The reason is that we only know the actions that have been taken by the agents at certain states (along the path). We have no information on their policies, and hence we may only be able to compute the cost at states not along the path.}

Then the DoR for each agent $i\in\mathcal{R}$ is defined as
\begin{equation}
    \phi_i = 
         \frac{1}{\left|\mathcal{R}\right|} \sum_{\mathcal{Y} \subseteq \mathcal{R} \backslash\{i\}} \frac{Q(\mathcal{Y} \cup\{i\})-Q(\mathcal{Y})}{\left(\begin{array}{c}
\left|\mathcal{R}\right|-1 \\
|\mathcal{Y}|
\end{array}\right)}.
\end{equation}
Since we have identified a subset of agents $\mathcal{R}$, computing Shapley value becomes less computational demanding than directly analyzing on the original MMDP.

\textcolor{blue}{The equation does not exactly match Eq.(4) because $Q(\mathcal{Y})$ punishes the deviation from the safe policy.}
